Knowledge is Power: Harnessing Large Language Models for Enhanced Cognitive Diagnosis

Cognitive Diagnosis Models (CDMs) are designed to assess students' cognitive states by analyzing their performance across a series of exercises. However, existing CDMs often struggle with diagnosing infrequent students and exercises due to a lack of rich prior knowledge. With the advancement in large language models (LLMs), which possess extensive domain knowledge, their integration into cognitive diagnosis presents a promising opportunity. Despite this potential, integrating LLMs with CDMs poses significant challenges. LLMs are not well-suited for capturing the fine-grained collaborative interactions between students and exercises, and the disparity between the semantic space of LLMs and the behavioral space of CDMs hinders effective integration. To address these issues, we propose a novel Knowledge-enhanced Cognitive Diagnosis (KCD) framework, which is a model-agnostic framework utilizing LLMs to enhance CDMs and compatible with various CDM architectures. The KCD framework operates in two stages: LLM Diagnosis and Cognitive Level Alignment. In the LLM Diagnosis stage, both students and exercises are diagnosed to achieve comprehensive and detailed modeling. In the Cognitive Level Alignment stage, we bridge the gap between the CDMs' behavioral space and the LLMs' semantic space using contrastive learning and mask-reconstruction approaches. Experiments on several real-world datasets demonstrate the effectiveness of our proposed framework.

==> tables/emb.tex <==
\begin{table}[ht]
\centering
 %Methods with `$^{*}$' means directly using ground truth review text in the testing phase, which are not feasible in practice.



\scalebox{0.9}{
\begin{tabular}{lcccc}
\toprule
LLM & Method &  AUC  & ACC & RMSE \\ \midrule
& NCD & 0.8256 & 0.7759 & 0.3926 \\ 
\midrule
\multirow{2}{*}{OpenAI}& NCD-Beh & 0.8422 &  0.7928 & 0.3781 \\
& NCD-Sem & 0.8460 & 0.7963 & 0.3764\\
\midrule
\multirow{2}{*}{Zhipu} &NCD-Beh &  0.8352 & 0.7873 & 0.3796\\
&NCD-Sem &  0.8365 & 0.7904 & 0.3776 \\
\midrule
\multirow{2}{*}{Tongyi} & NCD-Beh &  0.8387 & 0.7896 & 0.3792\\
&NCD-Sem & 0.8375  &0.7931  & 0.3768 \\
 


\bottomrule 
\end{tabular}}
\caption{Different LLMs on Linux dataset.}
\label{tab:emb}
\end{table}

==> tables/llm.tex <==
\begin{table}[ht]
\centering
 %Methods with `$^{*}$' means directly using ground truth review text in the testing phase, which are not feasible in practice.



\scalebox{0.9}{
\begin{tabular}{lcccc}
\toprule
LLM & Method &  AUC  & ACC & RMSE \\ \midrule
& NCD & 0.8256 & 0.7759 & 0.3926 \\ 
\midrule
\multirow{2}{*}{GPT-3.5-turbo}& NCD-Beh & 0.8422 &  0.7928 & 0.3781 \\
& NCD-Sem & 0.8460 & 0.7963 & 0.3764\\
\midrule
\multirow{2}{*}{GPT-4o-mini} &NCD-Beh &  0.8454 & 0.7963 & 0.3744\\
&NCD-Sem &  0.8491 & 0.7981 & 0.3715 \\
\midrule
\multirow{2}{*}{GLM-4} & NCD-Beh &  0.8432 & 0.7949 & 0.3758\\
&NCD-Sem &  0.8476 & 0.7975 & 0.3749 \\
 
 \midrule
\multirow{2}{*}{Qwen2.5-72B} & NCD-Beh &  0.8407 & 0.7912 & 0.3795\\
&NCD-Sem &  0.8415 & 0.7938 & 0.3772 \\

\midrule
\multirow{2}{*}{Qwen2.5-14B} & NCD-Beh &  0.8379 & 0.7882 & 0.3813\\
&NCD-Sem &  0.8381 & 0.7906 & 0.3794 \\

 
 \midrule
\multirow{2}{*}{Qwen2.5-coder-7B} & NCD-Beh &  0.8342 & 0.7834 & 0.3854\\
&NCD-Sem &  0.8367 & 0.7862 & 0.3825 \\

\bottomrule 
\end{tabular}}
\caption{Different LLMs on Linux dataset.}
\label{tab:llms}
\end{table}
